On Memory Codelets: Prefetching, Recoding, Moving and Streaming Data

For decades, memory capabilities have scaled up much slower than compute capabilities, leaving memory utilization as a major bottleneck. Prefetching and cache hierarchies mitigate this in applications with easily predictable memory accesses or those with high locality. In other applications like sparse linear algebra or graph-based applications, these strategies do not achieve effective utilization of memory. This is the case for the von Neumann model of computation, but other program execution models (PXM) provide different opportunities. Furthermore, the problem is complicated by increasing levels of heterogeneity and devices' varying memory subsystems. The Codelet PXM presented in this paper provides a program structure that allows for well-defined prefetching, streaming, and recoding operations to improve memory utilization and efficiently coordinate data movement with respect to computation. We propose the Memory Codelet, an extension to the original Codelet Model, to provide users these functionalities in a well-defined manner within the Codelet PXM.

==> outline.tex <==
\section*{Outline}
The idea is to provide a definition of memory codelets as an important element of the codelet pxm. We use it to demonstrate how memory codelet can help compute codelets have data in a format that makes sense for the computation.

Memory Codelets are Codelets that their purpose is not to heavily transform data through mathematical operations, but rather to prepare data into different formats that allows for more efficient computation. Memory Codelets are a general concept, but we will use the Sequential Codelet Model as the version of the Codelet PXM to explain the concept of memory Codelets. We will define equivalent operations to prefetching, and we will extend it to more complex patterns. Furthermore, we will discuss how memory codelets can be used to explicitly place memory near computation (percolation?), and also the use of memory codelets to recode data into formats that are more friendly to computation. We can provide multiple examples were memory codelets are useful, some inspired by architectures such as UDP, UAP, Takko, and others. 

Memory codelets do not need to be executed by CUs with heavy compute capabilities, instead they can be executed by memory managers, as used in the sequential Codelet Model. Memory codelets have been previously used (e.g. 2D memory access patters in the matrix multiplication example for SCM), but they have not been defined as in this paper. 

Contributions of this paper:
\begin{itemize}
    \item We provide a definition of a Memory codelet
    \item We provide an abstract machine that contains special memory compute units that are in charge of memory codelets and their scheduling decisions. Relate this to near memory compute
    \item We provide similes of memory Codelets with prefetching mechanism. A common prefetcher can be seen as a memory Codelet that performs streaming operations through a fifo queue. Likewise, memory codelets can be event driven Codelets that act on memory access patterns by applications, however, they are better used in conjunction with the application.
    \item We provide a set of example applications, and evaluate them in SCMUlate
    \item We can try to create a connection with pure misses and concurrent misses.
\end{itemize}

The structure of this paper is as follows:
\begin{itemize}
    \item Introduction: 
    \begin{itemize}
        \item Describe how there exists a lot of applications that cannot take advantage of caches and prefetching, due to different access patters. 
        \item Describe how others have aim to create special near memory compute architectures, but leaving the problem of the orchestration of computation and memory to the final user (e.g. offloading model).
        \item Use this section for background and related work due to page limitations
    \end{itemize}
    \item Memory codelets and abstract machine
    \begin{itemize}
        \item Define a memory codelet
        \item Describe an abstract machine that contains a memory unit, a CU that its purpose is to execute memory codelets. This CU can be extended with compute capabilities similar to UDP, takko or others.
        \item Describe an extension to the SCM used in the evaluation
        \item discuss prefetching, recoding, memory movement, and streaming through fifo queues
    \end{itemize}
    \item Evaluation
\begin{itemize}
    \item Create a hello world example for memory codelets. Likely one per type of memory codelet described above: e.g. tensor reshaping, or sparse matrix to dense matrix, or matrix transpose operation. Explain how it is possible to do prefetching through FIFO queues streaming. Explain how it is possible to use recoding through data transformation. 
    \item Create a complex problem: e.g. use the decompression evaluation done by P38 before in the context of UDP
    \item run these problem into the SCMulate
\end{itemize}
    \item Conclusions
    \item Papers to cite?
    \begin{itemize}
        \item UDP
        \item sparse papers w/ streaming (MetaStrider, OuterSPACE, SpArch, sparsecore?)
        \item Chiplets and the Codelet Model?
        \item Recode 10x10
        \item PIM papers
        \begin{itemize}
            \item SISA: Set-Centric Instruction Set Architecture
for Graph Mining on Processing-in-Memory Systems
            \item A Scalable Processing-in-Memory Accelerator for Parallel Graph Processing (note that this is PIM, not PNM)
            \item Tako A Polymorphic Cache Hierarchy for
General-Purpose Optimization of Data Movement
        \end{itemize}
        \item Related Work: Prodigy
    \end{itemize}
\end{itemize}

\begin{enumerate}
    \item Introduction
- Why memory is important, related work wrt architectures (e.g. near memory compute, recoding, application specific ...), but coordination is not there yet\\
1.1. Motivation and contributions:\\
- Offloading model is not great. Hard to reason about producer consumer, memory, and task coordination\\ 
- Codelet model lacks of explicite memory codelet model definition that comes with a different abstract machine \\
- Define contributions \\
- Case against coherency \\
\item Define PXM and introduce codelet model and sequential codelet model
\item Memory codelets. 
- Definition of memory codelets \\
- Abstract machine  \\
- Prefetching, streaming, recoding, and other elements that the runtime can do thanks to the codelet abstraction \\
\item Evaluation.
- Using SCMulate, we demonstrate how memory codelets can ease the memory usage. \\
- We have to think how to create an appropriate baseline (i.e. pointers only) \\
\item Conclusions.
\end{enumerate}
\newpage



